FasTUSS: Faster Task-Aware Unified Source Separation

Time-Frequency (TF) dual-path models are currently among the best performing audio source separation network architectures, achieving state-of-the-art performance in speech enhancement, music source separation, and cinematic audio source separation. While they are characterized by a relatively low parameter count, they still require a considerable number of operations, implying a higher execution time. This problem is exacerbated by the trend towards bigger models trained on large amounts of data to solve more general tasks, such as the recently introduced task-aware unified source separation (TUSS) model. TUSS, which aims to solve audio source separation tasks using a single, conditional model, is built upon TF-Locoformer, a TF dual-path model combining convolution and attention layers. The task definition comes in the form of a sequence of prompts that specify the number and type of sources to be extracted. In this paper, we analyze the design choices of TUSS with the goal of optimizing its performance-complexity trade-off. We derive two more efficient models, FasTUSS-8.3G and FasTUSS-11.7G that reduce the original model's operations by 81\% and 73\% with minor performance drops of 1.2~dB and 0.4~dB averaged over all benchmarks, respectively. Additionally, we investigate the impact of prompt conditioning to derive a causal TUSS model.

==> figs/maps/blind.tex <==
\matrix (m2) [
    matrix of math nodes,
    left delimiter={(},
    right delimiter={)},
    nodes={inner sep=0pt, outer sep=0pt, minimum size=0.7em, anchor=center},
    row sep=0.5em,
    column sep=0.5em,
    inner sep=0pt
] {
    1 & 0 & 0 & 0 & 0 \\
    0 & 1 & 0 & 0 & 0 \\
    1 & 1 & 1 & 1 & 1 \\
    1 & 1 & 1 & 1 & 1 \\
    1 & 1 & 1 & 1 & 1 \\
};

\draw[fill=\promptcolor] ([yshift=4pt]m2-1-1.north west) rectangle ++(\size, \size);
\draw[fill=\promptcolor] ([yshift=4pt]m2-1-2.north west) rectangle ++(\size, \size);
\draw[fill=\mixcolor] ([yshift=4pt]m2-1-3.north west) rectangle ++(\size, \size);
\draw[fill=\mixcolor] ([yshift=4pt]m2-1-4.north west) rectangle ++(\size, \size);
\draw[fill=\mixcolor] ([yshift=4pt]m2-1-5.north west) rectangle ++(\size, \size);

\draw[fill=\promptcolor] ([xshift=-15pt, yshift=-3.1pt]m2-1-1.west) rectangle ++(\size, \size);
\draw[fill=\promptcolor] ([xshift=-15pt, yshift=-3.1pt]m2-2-1.west) rectangle ++(\size, \size);
\draw[fill=\mixcolor] ([xshift=-15pt, yshift=-3.1pt]m2-3-1.west) rectangle ++(\size, \size);
\draw[fill=\mixcolor] ([xshift=-15pt, yshift=-3.1pt]m2-4-1.west) rectangle ++(\size, \size);
\draw[fill=\mixcolor] ([xshift=-15pt, yshift=-3.1pt]m2-5-1.west) rectangle ++(\size, \size);

\node [left=22pt of m2-3-1, yshift=7pt, rotate=90] {$\bm{Q}$};
\node [above=4pt of m2-1-3, yshift=7pt] {$\bm{K}$};

\draw [densely dashed] ([yshift=-2pt] m2-2-1.south west) -- ([yshift=-2pt] m2-2-5.south east);
\draw [densely dashed] ([xshift=2.25pt] m2-1-2.north east) -- ([xshift=2.25pt] m2-5-2.south east);

\node[below=2pt of m2] {\footnotesize (a) \texttt{BLINDPROMPT}};


==> figs/maps/causal.tex <==
\matrix (m) [
    right=30pt of m3,
    matrix of math nodes,
    left delimiter={(},
    right delimiter={)},
    nodes={inner sep=0pt, outer sep=0pt, minimum size=0.7em, anchor=center},
    row sep=0.5em,
    column sep=0.5em,
    inner sep=0pt
] {
    1 & 1 & 0 & 0 & 0\\
    1 & 1 & 0 & 0 & 0 \\
    1 & 1 & 1 & 0 & 0 \\
    1 & 1 & 1 & 1 & 0 \\
    1 & 1 & 1 & 1 & 1 \\
};

\draw[fill=\promptcolor] ([yshift=4pt]m-1-1.north west) rectangle ++(\size, \size);
\draw[fill=\promptcolor] ([yshift=4pt]m-1-2.north west) rectangle ++(\size, \size);
\draw[fill=\mixcolor] ([yshift=4pt]m-1-3.north west) rectangle ++(\size, \size);
\draw[fill=\mixcolor] ([yshift=4pt]m-1-4.north west) rectangle ++(\size, \size);
\draw[fill=\mixcolor] ([yshift=4pt]m-1-5.north west) rectangle ++(\size, \size);

\draw[fill=\promptcolor] ([xshift=-15pt, yshift=-3.1pt]m-1-1.west) rectangle ++(\size, \size);
\draw[fill=\promptcolor] ([xshift=-15pt, yshift=-3.1pt]m-2-1.west) rectangle ++(\size, \size);
\draw[fill=\mixcolor] ([xshift=-15pt, yshift=-3.1pt]m-3-1.west) rectangle ++(\size, \size);
\draw[fill=\mixcolor] ([xshift=-15pt, yshift=-3.1pt]m-4-1.west) rectangle ++(\size, \size);
\draw[fill=\mixcolor] ([xshift=-15pt, yshift=-3.1pt]m-5-1.west) rectangle ++(\size, \size);

\node [above=4pt of m-1-3, yshift=7pt] {$\bm{K}$};

\draw [densely dashed] ([yshift=-2pt] m-2-1.south west) -- ([yshift=-2pt] m-2-5.south east);
\draw [densely dashed] ([xshift=2.25pt] m-1-2.north east) -- ([xshift=2.25pt] m-5-2.south east);

\node[below=2pt of m] {\footnotesize (d) \texttt{CAUSAL}};


==> figs/maps/indall.tex <==
\matrix (m3) [
    right=30pt of m4,
    matrix of math nodes,
    left delimiter={(},
    right delimiter={)},
    nodes={inner sep=0pt, outer sep=0pt, minimum size=0.7em, anchor=center},
    row sep=0.5em,
    column sep=0.5em,
    inner sep=0pt
] {
    1 & 1 & 0 & 0 & 0 \\
    1 & 1 & 0 & 0 & 0 \\
    0 & 0 & 1 & 1 & 1 \\
    0 & 0 & 1 & 1 & 1 \\
    0 & 0 & 1 & 1 & 1 \\
};

\draw[fill=\promptcolor] ([yshift=4pt]m3-1-1.north west) rectangle ++(\size, \size);
\draw[fill=\promptcolor] ([yshift=4pt]m3-1-2.north west) rectangle ++(\size, \size);
\draw[fill=\mixcolor] ([yshift=4pt]m3-1-3.north west) rectangle ++(\size, \size);
\draw[fill=\mixcolor] ([yshift=4pt]m3-1-4.north west) rectangle ++(\size, \size);
\draw[fill=\mixcolor] ([yshift=4pt]m3-1-5.north west) rectangle ++(\size, \size);

\draw[fill=\promptcolor] ([xshift=-15pt, yshift=-3.1pt]m3-1-1.west) rectangle ++(\size, \size);
\draw[fill=\promptcolor] ([xshift=-15pt, yshift=-3.1pt]m3-2-1.west) rectangle ++(\size, \size);
\draw[fill=\mixcolor] ([xshift=-15pt, yshift=-3.1pt]m3-3-1.west) rectangle ++(\size, \size);
\draw[fill=\mixcolor] ([xshift=-15pt, yshift=-3.1pt]m3-4-1.west) rectangle ++(\size, \size);
\draw[fill=\mixcolor] ([xshift=-15pt, yshift=-2.1pt]m3-5-1.west) rectangle ++(\size, \size);

\node [above=4pt of m3-1-3, yshift=7pt] {$\bm{K}$};

\draw [densely dashed] ([yshift=-2pt] m3-2-1.south west) -- ([yshift=-2pt] m3-2-5.south east);
\draw [densely dashed] ([xshift=2.25pt] m3-1-2.north east) -- ([xshift=2.25pt] m3-5-2.south east);

\node[below=2pt of m3] {\footnotesize (c) \texttt{INDALL}};



==> figs/maps/indprompt.tex <==
\matrix (m4) [
    right=30pt of m2,
    matrix of math nodes,
    left delimiter={(},
    right delimiter={)},
    nodes={inner sep=0pt, outer sep=0pt, minimum size=0.7em, anchor=center},
    row sep=0.5em,
    column sep=0.5em,
    inner sep=0pt
] {
    1 & 1 & 0 & 0 & 0 \\
    1 & 1 & 0 & 0 & 0 \\
    1 & 1 & 1 & 1 & 1 \\
    1 & 1 & 1 & 1 & 1 \\
    1 & 1 & 1 & 1 & 1 \\
};

\draw[fill=\promptcolor] ([yshift=4pt]m4-1-1.north west) rectangle ++(\size, \size);
\draw[fill=\promptcolor] ([yshift=4pt]m4-1-2.north west) rectangle ++(\size, \size);
\draw[fill=\mixcolor] ([yshift=4pt]m4-1-3.north west) rectangle ++(\size, \size);
\draw[fill=\mixcolor] ([yshift=4pt]m4-1-4.north west) rectangle ++(\size, \size);
\draw[fill=\mixcolor] ([yshift=4pt]m4-1-5.north west) rectangle ++(\size, \size);

\draw[fill=\promptcolor] ([xshift=-15pt, yshift=-3.1pt]m4-1-1.west) rectangle ++(\size, \size);
\draw[fill=\promptcolor] ([xshift=-15pt, yshift=-3.1pt]m4-2-1.west) rectangle ++(\size, \size);
\draw[fill=\mixcolor] ([xshift=-15pt, yshift=-3.1pt]m4-3-1.west) rectangle ++(\size, \size);
\draw[fill=\mixcolor] ([xshift=-15pt, yshift=-3.1pt]m4-4-1.west) rectangle ++(\size, \size);
\draw[fill=\mixcolor] ([xshift=-15pt, yshift=-2.1pt]m4-5-1.west) rectangle ++(\size, \size);

\node [above=4pt of m4-1-3, yshift=7pt] {$\bm{K}$};

\draw [densely dashed] ([yshift=-2pt] m4-2-1.south west) -- ([yshift=-2pt] m4-2-5.south east);
\draw [densely dashed] ([xshift=2.25pt] m4-1-2.north east) -- ([xshift=2.25pt] m4-5-2.south east);

\node[below=2pt of m4] {\footnotesize (b) \texttt{INDPROMPT}};


